Data Formats in Analytical DBMSs: Performance Trade-offs and Future Directions

This paper evaluates the suitability of Apache Arrow, Parquet, and ORC as formats for subsumption in an analytical DBMS. We systematically identify and explore the high-level features that are important to support efficient querying in modern OLAP DBMSs and evaluate the ability of each format to support these features. We find that each format has trade-offs that make it more or less suitable for use as a format in a DBMS and identify opportunities to more holistically co-design a unified in-memory and on-disk data representation. Notably, for certain popular machine learning tasks, none of these formats perform optimally, highlighting significant opportunities for advancing format design. Our hope is that this study can be used as a guide for system developers designing and using these formats, as well as provide the community with directions to pursue for improving these common open formats.

==> compression.tex <==
\subsection{Data Encoding and Compression}

Data system employ compression algorithms to reduce the data size and improve bandwidth utilization. compression is important for organizations storing data in public clouds. So good compression really matters in terms of saving cost. Conventional compression focus on reducing the file size. But when there come the queries. Improper compression may hurt the query performance. As some compression require decompression before we can apply the queries. Which waste a lot of computation resources and optimization opportunity. A good compression should also be able to support query directly on the compressed data, and even boost the query performance.
There has been many compression approaches proposed to achieve the purpose of making data smaller and query faster. 

% Databases use compression methods to reduce storage size and get better utilization of bandwidth. Besides, compression methods may affect query performance. Some require decompression before query and can worsen query performance. Some allow in-situ queries and data skipping, thus improve query performance.


\subsubsection{Encodings}
Byte-oriented compression, such as Gzip and Snappy are widely used for data compression. They are applicable to all type of data, and in general has a good compression ratio.  But these methods are computationally intensive.  Every time we execute a query, we need to decompress a whole data block. This takes a considerable amount of time.

Columnar databases store data of the same type together, allowing us to use lightweight encodings for compression.
Lightweight Encodings are often designed to compress only one specific type of datasets. They encode and decode data fast. Some encodings also support in-situ queries and data skipping to improve query performance. Here we give a brief of several popular lightweight encoding algorithms and their applicable scenarios.

\textbf{Bit-Packed Encoding (BP)} works on integer data. It finds the minimal number of bits needed to represent the numbers and removes excessive leading zeros. It works best when the target numbers have similar bit-width.

\textbf{Dictionary encoding }works on all types of data. It encodes each distinct entry in the dataset with an integer key, and bit-packs the integers. Dictionary encoding works best when the dataset has small cardinality and large number of repetitions.

\textbf{Run-length encoding (RLE)} works on data with many consecutive repetitions. It replaces a run of same value with a pair of value and how many times it is repeated.

\textbf{Delta encoding} works on integer data. It stores the delta between numbers and bit-pack the deltas. It works best when the numbers are large, but delta between numbers are small.

These are a basic set of encoding algorithms and there are also variations and hybrid version derived from them.

\subsubsection{Direct Query}
\todo{Abadi paper, redshift, sql sever}

\subsubsection{Compression}

\todo{Compression Gzip, Snappy, LZ4, zlib}

==> compute.tex <==
\section{Arrow Compute}

\todo{Hopefully we'll grab the Weld code and run experiments using its original format and compare to Arrow.  Ideally we'll do this with an ablation study that turns on/off combinations of optimizations (e.g. SIMD) to see the effect of each optimization on each format. }

\AP {Gandiva parameters}

\AP {Detected CPU Name : skylake-avx512.}

\AP {Detected CPU Features: +sse2 +cx16 +sahf -tbm -avx512ifma -sha -gfni -fma4 -vpclmulqdq +prfchw +bmi2 -cldemote +fsgsbase -ptwrite +xsavec +popcnt +aes -avx512bitalg -movdiri +xsaves -avx512er -avx512vnni -avx512vpopcntdq -pconfig -clwb +avx512f -clzero -pku +mmx -lwp -rdpid -xop +rdseed -waitpkg -movdir64b -sse4a +avx512bw +clflushopt +xsave -avx512vbmi2 +64bit +avx512vl +invpcid +avx512cd +avx -vaes +cx8 +fma +rtm +bmi -enqcmd +rdrnd -mwaitx +sse4.1 +sse4.2 +avx2 +fxsr -wbnoinvd +sse +lzcnt +pclmul -prefetchwt1 +f16c +ssse3 -sgx -shstk +cmov -avx512vbmi -avx512bf16 +movbe +xsaveopt +avx512dq +adx -avx512pf +sse3.}


\AP{target datalayout = "e-m:e-p270:32:32-p271:32:32-p272:64:64-i64:64-f80:128-n8:16:32:64-S128", where e mean bytes in memory are stored using little endian schema, m:e - ELF name mangling is used. p270:32:32 - alignment in data, given in bits. n specifies which native register sizes are available (8-bit , 16-bit, 32-bit and 64-bit wide registers are natively supported). S128 means that the stack maintains a 16-byte alignment. target triple = "x86\_64-pc-linux-gnu" - architecture we're compiling for.
}

==> discussion.tex <==
\section{Discussion}

==> format.tex <==
\section{Arrow Format}

\todo{Performance characteristics of Arrow vs other formats (Parquet, Feather, ORC, AVRO, etc.)}

For decades, many data engines used row-oriented storage formats for OLTP query workloads. As more complex workload focusing on only few attributes becomes the trend, columnar storage format is more viable. In the big data environments, there are various optimized data formats for data storage and computation: Parquet, Feather, ORC, AVRO, etc. These data formats share some similarities and provide some degree of compression. Each format has its own pros and cons depending on the use cases and exists to serve one or several purposes.


\begin{table*}[h]
\centering
\caption{Data format comparison \todo{add supported systems} }
\label{tab:format}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{ } & encoding & compression & row/column & index & storage & computation & systems\\ \hline
\textbf{Arrow} & null & null & column & \checkmark & $\times$ & \checkmark  & \\ \hline
\textbf{Feather} & DICT & ZSTD,LZ4 & column & \checkmark & \checkmark & $\times$   &\\ \hline
\textbf{Parquet} & DICT,RLE,BP & gzip, snappy, ZSTD, LZ4 & column & \checkmark & \checkmark & $\times$ & Spark, Presto\\ \hline
\textbf{ORC} & DICT,RLE,BP & snappy, zlib, LZ4 & column & \checkmark & \checkmark & $\times$ & Hive, Presto\\ \hline
\textbf{Avro} & DICT,RLE,BP & gzip, snappy, ZSTD, LZ4 & row & \checkmark & \checkmark & $\times$ & Kafka\\ \hline
\end{tabular}
% \vspace{--10pt}
\end{table*}

\subsection{Arrow}
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.40]{figures/arrow.pdf}
    \caption{Arrow Format}
    \label{fig:arrow}
\end{figure}
Arrow \cite{arrow} is a columnar data structure supporting efficient in-memory computing. It is able to represent flat and hierarchical data for efficient analytic operations on modern CPU and GPU hardware. Arrow is designed to be complementary to the popular on-disk columnar data formats Parquet and ORC for efficiently processing data in-memory. Those on-disk data file can be decompressed, decoded and then loaded  into Arrow in-memory columnar data structures, so the analytics can be applied on the decoded in-memory data structure. Arrow columnar format has some nice properties: random access is O(1) and each value cell is next to the previous and following one in memory, so it's efficient to iterate over. 
Arrow defines a binary serialization protocol for converting a collection of Arrow record batch that can be used for messaging, interprocess communication, and saving Arrow blob into storage. The deserialization of arrow blob pays effectively zero cost with memory-mapping.
Arrow only support lightweight dictionary encoding (and, dictionary encoding is for string and binary only), it can be further compressed by Arrow Feather \cite{feather} with ZSTD or LZ4 compression.

\subsection{Feather}
\begin{figure}[!t]
    \centering
    \adjustbox{margin=1em,width=\linewidth,set height=2.5cm,set depth=2.5cm,frame,center}{Feather}
    \caption{Arrow Feather Format}
    \label{fig:feather}
\end{figure}
Feather is a column-oriented binary disk-based format based on Apache Arrow. Feather was designed for for fast, language-agnostic data frame storage. It provides light-weight encoding and some compression approaches for space efficiency. There are two version for Feather
Feather version 1 (V1) and version 2 (V2). V2 is the default version for now with support of storing all Arrow data types and it is an exactly representation of Arrow IPC format with general purpose compression support. V1 is a legacy version with less Arrow data types supported and no compression support. In our work, we focus on Feather V2 only.

\subsection{Parquet}

\begin{figure}[t]
\centering
\begin{tikzpicture}
[
scale=0.5,
every node/.style={scale=0.5},
block/.style={draw=gray,fill=gray!20!white},
column/.style={fill=gray!30!white,minimum width=1.5cm, minimum height=1cm},
page/.style={fill=gray!40,draw=gray,minimum height=0.8cm}
]
\draw[gray,fill=gray!10!white](-1.5,2) to (5.5,2) to
(5.5,-2) .. controls (3,-1.8) and (0,-2.5) .. (-1.5,-2) -- cycle;

\draw[gray,fill=gray!10!white]
(5.5,-2.5) .. controls (3,-2.3) and (0,-3) .. (-1.5,-2.5)
to (-1.5,-4.8) to (5.5,-4.8) -- cycle;

\node[block, minimum width =6cm, minimum height= 2cm] at (2,0.2) {};
\node at (2,0.9) {Row Group 1};
\node[block,column] at (0,0){Col 1};
\node[block,column] at (1.75,0){Col 2};
\node at (2.9,0){$\hdots$};
\node[block,column] at (4,0){Col n};
\node[block,scale=0.7]at(4,0.9) {Zone Map};

\node[block, minimum width=6cm,minimum height=0.8cm] at (2,-1.4) {Row Group 2};
\node at (2,-2.3) {$\vdots$};
\node[block, minimum width=6cm,minimum height=0.8cm] at (2,-3.3) {Row Group m};
\node[block, fill=gray!10, minimum width=7cm,minimum height=1cm] at (2,-4.6)
{File Footer (contains metadata)};
\node at (2,1.6) {Parquet File};

\node[block,minimum width=3cm,minimum height=4cm] at (-3,0) {Column};
\node[page] at(-3,1.3) {Dictionary Page};
\node[page] at(-3,0.2) {Data Page 1};
\node at (-3,-0.5) {$\vdots$};
\node[page] at(-3,-1.4) {Data Page K};

\draw[dashed,gray] (-2,2) to (-0.7,0.5);
\draw[dashed,gray] (-2,-2) to (-0.7,-0.5);

\end{tikzpicture}
\caption{Parquet Columnar Store Format}
\label{fig:parquet}
\end{figure}
Parquet \cite{parquet} is a columnar-oriented storage file format inspired from the nested data storage format outlined in the Google Dremel \cite{melnik2010dremel}. Parquet is designed to make the advantages of compressed, efficient columnar data representation available to many data processing systems in the Hadoop ecosystem. Parquet integrates with many efficient compression and encoding approaches to achieve space-efficient layout.
As shown in Figure \ref{fig:parquet}, a Parquet file is made up of several row groups, which are indexed by block metadata saved in a file footer. A row group consists of several column chunks with metadata also in the file footer. In each column chunk, there are compressed data pages and a dictionary page if dictionary encoding enabled. The dictionary is stored in a dictionary page per column chunk. Columns are aligned in row group level, which means all data for a given row is organized in the same row group. In the file footer metadata is organized about column chunk metadata, zone maps (e.g. min, max and number of nulls), encoding, and compression information. Parquet always applies dictionary encoding for all supported types but it fall back to plain encoding or other custom encoding when dictionary is larger than a predefined threshold (number of entries, dictionary size). Parquet is designed to be space and IO-efficient at the expense of CPU utilization for decoding. It does not provide any data structures for in-memory computing. Even with the newly added "index page" to facilitate the access of data entries, Parquet's random access operation are still costly in general.

\subsection{ORC}

Optimized Row Columnar (ORC) \cite{orc} is a column-oriented storage format designed for Hadoop workloads. ORC stores metadata with Protocol Buffers allowing addition and removal of data fields.
ORC files contain groups of row data called stripes, along with auxiliary information in a file footer. At the end of the file, a postscript holds compression parameters and the size of the compressed footer. ORC is  optimized for read-heavy analytical workloads. The default stripe size is 250 MB. Large stripe sizes enable large efficient reads from HDFS. Stripe is the basic unit for a batch of row data, which is further split into streams physically. ORC organizes a given column in separate index, present and data stream depending on the encoding approach. It also provides index and present stream in the row level for fast query and null check. ORC also supports dictionary encoding for string data type. Similar to Parquet, ORC fall back to direct encoding when the ratio of distinct value over number of records greater than the given threshold (0.8 in hive setting). 
\begin{figure}[!t]
    \centering
    \adjustbox{margin=1em,width=\linewidth,set height=2.5cm,set depth=2.5cm,frame,center}{ORC}
    \caption{ORC Format}
    \label{fig:orc}
\end{figure}

\subsection{Avro}
\begin{figure}[!t]
    \centering
    \adjustbox{margin=1em,width=\linewidth,set height=2.5cm,set depth=2.5cm,frame,center}{Avro}
    \caption{Avro Format}
    \label{fig:avro}
\end{figure}
Avro is a row-oriented storage format. Avro stores data schema as JSON in the header of file so that it's excellent for schema evolution tasks and ideal for write heavy data operations such as entire row consumption and processing. Avro also supports serialization and RPC framework with block level compression.

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{} & \textbf{int} & \textbf{double} & \textbf{string} & \textbf{decimal} \\ \hline
\textbf{parquet} & dict-RLE & dict-RLE & dict-RLE & - \\ \hline
\textbf{arrow-feather} & null  & null & dict & null  \\ \hline
\textbf{orc} & RLE & Plain & dict-RLE & Int-RLE \\ \hline
\end{tabular}
\caption{Encoding comparison}
\label{tab:format-compare}
\end{table}

Arrow feather defines identical compression for data arrays in the same record batch, while Parquet provides different custom codec for the columnchunks in the same rowgroup. The flexibility of using custom codec for given data unit makes it possible for auto encoding and compression selection based on the data features and future workload \cite{jiang2021good}.

==> include/vldb.tex <==
%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbdoi{10.14778/3611479.3611507}
\newcommand\vldbpages{3044 - 3056}
% issue-specific
\newcommand\vldbvolume{16}
\newcommand\vldbissue{11}
\newcommand\vldbyear{2023}
% should be fine as it is
\newcommand\vldbauthors{\authors}
% \newcommand\vldbauthors{Chunwei Liu, Anna Pavlenko, Matteo Interlandi, and Brandon Haynes}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{https://github.com/Tranway1/ColumnarFormatsEval}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{empty} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%


==> taxonomy.tex <==
\section{Taxonomy of Arrow Systems}

\todo{Taxonomy of DBMSs and how they use Arrow (end-to-end, transcode at IO, partial internal support): mini qualitative survey}

\todo{Types of optimizations applied to Arrow (SIMD, prefetching, pipelining(operator fusion), compressed domain, native code, zero copy ? , Arrow Flight.)}

\todo{Arrow variants, heterogeneous hardware?}


Arrow adoption goals [Vectorized Query Processing using Apache Arrow
Strata Data Conference, San Jose
March 7, 2018
Siddharth Teotia]:
\begin{itemize}
    \item Columnar in-memory representation optimized for efficient use of processor cache through data locality.
    \item Take advantage of modern CPU characteristics by implementing algorithms that leverage hardware acceleration.
    \item Interoperability for high speed exchange between data
systems.
    \item Can be embedded in execution engines, storage layers, etc.
    \item “Flight” protocol is designed to enable Arrow data to be streamed efficiently
\end{itemize}

Arrow-native or compatible
\begin{itemize} 

    \item  \textit{DataFusion} - an extensible query execution framework, written in Rust, that uses Apache Arrow as its in-memory format. DataFusion supports both an SQL and a DataFrame API for building logical query plans as well as a query optimizer and execution engine \cite{datafusion}.
    \item  cuDF (from RAPIDS data science framework) is a Python GPU DataFrame library (built on the Apache Arrow columnar memory format) for loading, joining, aggregating, filtering, and otherwise manipulating data. \cite{cuDF}
 
    \item  \textit{Gandiva} - LLVM-based execution kernel built on top of Apache Arrow format \cite{gandiva}. Gandiva is used for accelerating computations via vectorization. ALICE Run 3 Analysis Framework built by CERN has achieved throughput boost 3-10 times after integration of Apache Arrow and Gandiva \cite{Alkin2021ALICER3}.    
    \item  \textit{Dremio} SQL Data Platform is based on Apache Arrow as internal format, utilizes Arrow Compute Kernels and Gandiva to accelerate data processing. \cite{dremio}
    \item \textit{Ballista} [not in production] is a distributed compute platform primarily implemented in Rust, and powered by Apache Arrow and DataFusion. The combination of Rust and Arrow provides excellent memory efficiency and memory usage can be 5x - 10x lower than Apache Spark in some cases, which means that more processing can fit on a single node, reducing the overhead of distributed compute \cite{ballista}. 
\item \textit{NoisePage} \cite{li2020mainlining} - first transactional system, which utilizes Apache Arrow natively . The main challenge with using columnar formats is their optimizations for read/append operations and write amplification. NoisePage uses relaxed Arrow format (which is a generalization of original Arrow format) with lightweight transformation operation after to put cold data into full Arrow. Using Apache Arrow as internal format allows NoisePage to export data to external analytical tools at zero serialization overhead .  
 \end{itemize}
    \item Native Engine for Spark SQL is designed to reimplement Spark SQL execution layer via using Apache Arrow format for data, Arrow Compute Kernels and Gandiva for computations. 

 C-Data Interface (zero copy benefits)
 \begin{itemize} 
    \item DuckDB
    \item Velox - open-source C++ database vectorized acceleration library by Meta (Facebook). It's using arrow-compatible columnar memory layout module and features Expression Eval - a fully vectorized expression evaluation engine that allows expressions to be efficiently executed on top of Vector/Arrow encoded data.\cite{velox}
  \end{itemize}

 Arrow-supported
 \begin{itemize} 
    \item BigQuery
    \item Snowflake
    
    \item ClickHouse \url{https://clickhouse.com/docs/en/interfaces/formats/}
    
    \item Spark \url{https://spark.apache.org/docs/3.0.1/sql-pyspark-pandas-with-arrow.html\#apache-arrow-in-spark}:  used in Spark to efficiently transfer data between JVM and Python processes.Arrow is available as an optimization when converting a Spark DataFrame to a Pandas DataFrame using the call toPandas() and when creating a Spark DataFrame from a Pandas DataFrame. Pandas UDFs are user defined functions that are executed by Spark using Arrow to transfer data and Pandas to work with the data, which allows vectorized operations.  
    \item  OmniSci (formerly MapD): In-memory columnar SQL engine designed to run on both GPUs and CPUs. OmniSci supports Arrow for data ingest and data interchange via CUDA IPC handles. This work is part of the GPU Open Analytics Initiative
    \item AWS Wrangler 
 
\end{itemize}

Arrow-based tooling
 \begin{itemize} 
    \item Turbodbc: Python module to access relational databases via the Open Database Connectivity (ODBC) interface. It provides the ability to return Arrow Tables and RecordBatches in addition to the Python Database API Specification 2.0.
    \item Substrait - collection of objects that model abstract analytics. Cross-Language Serialization for Relational Algebra on top of Apache Arrow. 
    \item pyarrow 
 \end{itemize}
